A Max-Flow Min-Cut Theorem for Quantum Graphs

We propose natural definitions of cuts and flows for quantum graphs. For cuts we consider two notions: ordinary cuts, which partition the vertex set into two parts; and generalised cuts, defined as a continuous relaxation of the binary partition function. We show that our definitions satisfy a max-flow min-cut theorem: For any disjoint terminal sets $S$ and $T$, the maximum value of an $S$-$T$-flow of a quantum graph equals the minimum value of a generalised $S$-$T$ cut, while the minimum value of an ordinary $S$-$T$ cut can be larger. While for classical graphs the values of the minimum generalised cut and the minimum ordinary cut coincide---recovering the classical max-flow min-cut theorem---we also show how it is more natural to think of flows as duals of generalised cuts instead of ordinary cuts.

==> style/shapes.tex <==
\makeatletter
\pgfkeys{/pgf/apex angle/.initial=110}

\pgfdeclareshape{cut triangle up}{
    \savedanchor\centerpoint{\pgfpointorigin}
    
    \savedanchor\dimensions{
        \pgfmathsetlength\pgf@x{.5 * \pgfkeysvalueof{/pgf/minimum width}}
        \pgfmathsetmacro{\theta}{\pgfkeysvalueof{/pgf/apex angle}}
        \pgfmathsetlength\pgf@y{\pgf@x / tan(\theta/2)}
        \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/inner xsep}}
        \pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/inner ysep}}
        \pgfpoint{\pgf@x}{\pgf@y}
    }

    \anchor{text}{\pgfpoint{-.4\wd\pgfnodeparttextbox}{-.4\ht\pgfnodeparttextbox}}

    \anchor{center}{\centerpoint}
    \anchor{north}{\dimensions \pgfpoint{0pt}{\pgf@y}}
    \anchor{south}{\dimensions \pgfpoint{0pt}{-\pgf@y}}
    \anchor{west}{\dimensions \pgfpoint{-\pgf@x}{-\pgf@y}}
    \anchor{east}{\dimensions \pgfpoint{\pgf@x}{-\pgf@y}}
    
    \backgroundpath{
        \dimensions
        \pgf@xa=\pgf@x \pgf@ya=\pgf@y
        
        % Define the horizontal inset of the vertical cut
        \pgfmathsetmacro{\cutwidth}{0.4 * \pgf@xa} 
        \pgfmathsetmacro{\shift}{0.0 * \cutwidth}       
        \pgfmathsetmacro{\yshift}{0.5 * \cutwidth}       
        
        % Calculate the Y-coordinate where the vertical cut hits the right slope
        % This keeps the vertex on the original triangle boundary
        \pgfmathsetmacro{\yintersect}{-\pgf@ya + (2 * \pgf@ya * \cutwidth / \pgf@xa)}

        % 1. Start at the Apex (Top)
        \pgfpathmoveto{\pgfpoint{0pt - \shift}{\pgf@ya+\yshift}}
        % 2. Line to Bottom Left
        \pgfpathlineto{\pgfpoint{\pgf@xa-\shift}{-\pgf@ya+\yshift}}
        % 3. Line to the start of the vertical cut (Bottom Right)
        \pgfpathlineto{\pgfpoint{-\pgf@xa + \cutwidth-\shift}{-\pgf@ya+\yshift}}
        % 4. Vertical line up to the intersection with the right slope
        \pgfpathlineto{\pgfpoint{-\pgf@xa + \cutwidth-\shift}{\yintersect+\yshift}}
        % 5. Close back to Apex
        \pgfpathclose
    }
}

\pgfdeclareshape{cut triangle down}{
    \savedanchor\centerpoint{\pgfpointorigin}
    
    \savedanchor\dimensions{
        \pgfmathsetlength\pgf@x{.5 * \pgfkeysvalueof{/pgf/minimum width}}
        \pgfmathsetmacro{\theta}{\pgfkeysvalueof{/pgf/apex angle}}
        \pgfmathsetlength\pgf@y{\pgf@x / tan(\theta/2)}
        \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/inner xsep}}
        \pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/inner ysep}}
        \pgfpoint{\pgf@x}{\pgf@y}
    }

    \savedanchor\textsize{
        \pgf@x=.5\wd\pgfnodeparttextbox
        \pgf@y=.5\ht\pgfnodeparttextbox
    }

    \anchor{text}{\pgfpoint{-.4\wd\pgfnodeparttextbox}{-.4\ht\pgfnodeparttextbox}}

    \anchor{center}{\centerpoint}
    \anchor{north}{\dimensions \pgfpoint{0pt}{\pgf@y}}
    \anchor{south}{\dimensions \pgfpoint{0pt}{-\pgf@y}}
    \anchor{west}{\dimensions \pgfpoint{-\pgf@x}{-\pgf@y}}
    \anchor{east}{\dimensions \pgfpoint{\pgf@x}{-\pgf@y}}
    
    \backgroundpath{
        \dimensions
        \pgf@xa=\pgf@x \pgf@ya=\pgf@y
        
        % Define the horizontal inset of the vertical cut
        \pgfmathsetmacro{\cutwidth}{0.4 * \pgf@xa} 
        \pgfmathsetmacro{\shift}{0.0 * \cutwidth}       
        \pgfmathsetmacro{\yshift}{0.5 * \cutwidth}       

        % Calculate the Y-coordinate where the vertical cut hits the right slope
        % This keeps the vertex on the original triangle boundary
        \pgfmathsetmacro{\yintersect}{-\pgf@ya + (2 * \pgf@ya * \cutwidth / \pgf@xa)}

        % 1. Start at the Apex (Top)
        \pgfpathmoveto{\pgfpoint{0pt - \shift}{-\pgf@ya-\yshift}}
        % 2. Line to Bottom Left
        \pgfpathlineto{\pgfpoint{\pgf@xa - \shift}{\pgf@ya-\yshift}}
        % 3. Line to the start of the vertical cut (Bottom Right)
        \pgfpathlineto{\pgfpoint{-\pgf@xa + \cutwidth - \shift}{\pgf@ya-\yshift}}
        % 4. Vertical line up to the intersection with the right slope
        \pgfpathlineto{\pgfpoint{-\pgf@xa + \cutwidth - \shift}{-\yintersect-\yshift}}
        % 5. Close back to Apex
        \pgfpathclose
    }
}

\pgfdeclareshape{cut triangle up alt}{
    \savedanchor\centerpoint{\pgfpointorigin}
    
    \savedanchor\dimensions{
        \pgfmathsetlength\pgf@x{.5 * \pgfkeysvalueof{/pgf/minimum width}}
        \pgfmathsetmacro{\theta}{\pgfkeysvalueof{/pgf/apex angle}}
        \pgfmathsetlength\pgf@y{\pgf@x / tan(\theta/2)}
        \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/inner xsep}}
        \pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/inner ysep}}
        \pgfpoint{\pgf@x}{\pgf@y}
    }

    \anchor{text}{\pgfpoint{-.4\wd\pgfnodeparttextbox}{-.4\ht\pgfnodeparttextbox}}

    \anchor{center}{\centerpoint}
    \anchor{north}{\dimensions \pgfpoint{0pt}{\pgf@y}}
    \anchor{south}{\dimensions \pgfpoint{0pt}{-\pgf@y}}
    \anchor{west}{\dimensions \pgfpoint{-\pgf@x}{-\pgf@y}}
    \anchor{east}{\dimensions \pgfpoint{\pgf@x}{-\pgf@y}}
    
    \backgroundpath{
        \dimensions
        \pgf@xa=\pgf@x \pgf@ya=\pgf@y
        
        % Define the horizontal inset of the vertical cut
        \pgfmathsetmacro{\cutwidth}{0.4 * \pgf@xa} 
        \pgfmathsetmacro{\shift}{0.0 * \cutwidth}       
        \pgfmathsetmacro{\yshift}{0.5 * \cutwidth}       
        
        % Calculate the Y-coordinate where the vertical cut hits the right slope
        % This keeps the vertex on the original triangle boundary
        \pgfmathsetmacro{\yintersect}{-\pgf@ya + (2 * \pgf@ya * \cutwidth / \pgf@xa)}

        % 1. Start at the Apex (Top)
        \pgfpathmoveto{\pgfpoint{0pt + \shift}{\pgf@ya+\yshift}}
        % 2. Line to Bottom Left
        \pgfpathlineto{\pgfpoint{-\pgf@xa+\shift}{-\pgf@ya+\yshift}}
        % 3. Line to the start of the vertical cut (Bottom Right)
        \pgfpathlineto{\pgfpoint{\pgf@xa - \cutwidth+\shift}{-\pgf@ya+\yshift}}
        % 4. Vertical line up to the intersection with the right slope
        \pgfpathlineto{\pgfpoint{\pgf@xa - \cutwidth+\shift}{\yintersect+\yshift}}
        % 5. Close back to Apex
        \pgfpathclose
    }
}

\pgfdeclareshape{cut triangle down alt}{
    \savedanchor\centerpoint{\pgfpointorigin}
    
    \savedanchor\dimensions{
        \pgfmathsetlength\pgf@x{.5 * \pgfkeysvalueof{/pgf/minimum width}}
        \pgfmathsetmacro{\theta}{\pgfkeysvalueof{/pgf/apex angle}}
        \pgfmathsetlength\pgf@y{\pgf@x / tan(\theta/2)}
        \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/inner xsep}}
        \pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/inner ysep}}
        \pgfpoint{\pgf@x}{\pgf@y}
    }

    \savedanchor\textsize{
        \pgf@x=.5\wd\pgfnodeparttextbox
        \pgf@y=.5\ht\pgfnodeparttextbox
    }

    \anchor{text}{\pgfpoint{-.4\wd\pgfnodeparttextbox}{-.4\ht\pgfnodeparttextbox}}

    \anchor{center}{\centerpoint}
    \anchor{north}{\dimensions \pgfpoint{0pt}{\pgf@y}}
    \anchor{south}{\dimensions \pgfpoint{0pt}{-\pgf@y}}
    \anchor{west}{\dimensions \pgfpoint{-\pgf@x}{-\pgf@y}}
    \anchor{east}{\dimensions \pgfpoint{\pgf@x}{-\pgf@y}}
    
    \backgroundpath{
        \dimensions
        \pgf@xa=\pgf@x \pgf@ya=\pgf@y
        
        % Define the horizontal inset of the vertical cut
        \pgfmathsetmacro{\cutwidth}{0.4 * \pgf@xa} 
        \pgfmathsetmacro{\shift}{0.0 * \cutwidth}       
        \pgfmathsetmacro{\yshift}{0.5 * \cutwidth}       

        % Calculate the Y-coordinate where the vertical cut hits the right slope
        % This keeps the vertex on the original triangle boundary
        \pgfmathsetmacro{\yintersect}{-\pgf@ya + (2 * \pgf@ya * \cutwidth / \pgf@xa)}

        % 1. Start at the Apex (Top)
        \pgfpathmoveto{\pgfpoint{0pt + \shift}{-\pgf@ya-\yshift}}
        % 2. Line to Bottom Left
        \pgfpathlineto{\pgfpoint{-\pgf@xa + \shift}{\pgf@ya-\yshift}}
        % 3. Line to the start of the vertical cut (Bottom Right)
        \pgfpathlineto{\pgfpoint{\pgf@xa - \cutwidth + \shift}{\pgf@ya-\yshift}}
        % 4. Vertical line up to the intersection with the right slope
        \pgfpathlineto{\pgfpoint{\pgf@xa - \cutwidth + \shift}{-\yintersect-\yshift}}
        % 5. Close back to Apex
        \pgfpathclose
    }
}
\makeatother

